Localization theory for derivators

We outline the theory of reflections for prederivators, derivators and stable derivators. In order to parallel the classical theory valid for categories, we outline how reflections can be equivalently described as categories of fractions, reflective factorization systems, and categories of algebras for idempotent monads. This is a further development of the theory of monads and factorization systems for derivators.

==> sections/04-preslim.tex <==
% %!TEX root = ../localization.tex
% % \section{Preservation, reflection, and creation of co/limits}
% % \label{sec:preslim}
% % In order to discuss the interaction of limits and reflections more systematically, we include the following definition.

% % \begin{defn}\label{defn:refl}
% % Let $F\colon\D\to\E$ be a morphism of derivators and let $u\colon A\to B$ be in $\cCat$.
% % \begin{enumerate}
% % \item The morphism $F$ \textbf{reflects left} (resp. \textbf{right}) \textbf{Kan extensions along $u$} if for every diagram $X\in\D(B)$ such that $FX\in\E(B)$ lies in the essential image of $u_!\colon\E(A)\to\E(B)$ (resp., of $u_*\colon\E(A)\to\E(B)$) then already $X$ lies in the essential image of $u_!\colon\D(A)\to\D(B)$ (resp., of $u_*\colon\D(A)\to\D(B)$).
% % \item The morphism $F$ \textbf{reflects colimits of shape $A$} if it reflects left Kan extensions along $A\to A^\rhd$ (resp., $A \to A^\lhd$).
% % \end{enumerate} 
% % \end{defn}
% % \begin{rmk}
% % \begin{enumerate}
% % \item A morphism $F$ of derivators reflects left Kan extensions along $u$ if and only if the opposite morphism $F\op$ reflects right Kan extensions along $u\op$.
% % \item Let $F\colon\cC\to\cD$ be a functor between complete and cocomplete categories. Then $F$ reflects colimits of shape $A$ if and only if $y_F$ preserves colimits of shape $A$. In fact, it suffices to note that $X\colon A^\rhd\to\cC$ is a colimiting cocone if and only if it lies in the essential image of the left Kan extension along $i_A\colon A\to A^\rhd$.
% % \end{enumerate}
% % \end{rmk}

% % \begin{rmk}\label{rmk:pres-refl-colim}
% % By \cite[Prop.~3.9]{groth:revisit} the following are equivalent for a morphism $F\colon\D\to\E$ of derivators and $A\in\cCat$.
% % \begin{enumerate}
% % \item The morphism $F$ preserves and reflects colimits of shape $A$. 
% % \item A cocone $X\in\D(A^\rhd)$ is colimiting if and only if the cocone $FX\in\E(A^\rhd)$ is colimiting.
% % \end{enumerate}
% % \end{rmk}

% % \begin{defn}\label{defn:cons}
% % A morphism of prederivators is \textbf{conservative} if every component is conservative.
% % \end{defn}

% % Thus, a morphism $F\colon\D\to\E$ is conservative if a morphism $f\colon X\to Y$ in $\D(A)$ is an isomorphism as soon as $Ff\colon FX\to FY$ is an isomorphism in $\E(A)$.

% % \begin{egs}\leavevmode\label{egs:ff-cons}
% % Fully faithful morphism of prederivators are conservative. In particular, reflections, coreflections, and equivalences are conservatice.
% % \end{egs} 

% % For conservative morphisms there is the following connection between preservation and reflection of Kan extensions along fully faithful functors.

% \begin{lem}\label{lem:cons-refl}
% Let $F\colon\D\to\E$ be a conservative morphism of derivators and let $u\colon A\to B$ be fully faithful. If $F$ preserves left Kan extensions along $u$, then $F$ reflects left Kan extensions along $u$.
% \end{lem}
% \begin{proof}
% Since $u\colon A\to B$ is fully faithful, the same is true for the left Kan extension functors $u_!$ in $\D$ and $\E$, and we can hence characterize the respective essential images by the invertibility of the counits $\varepsilon\colon u_! u^\ast\to\id$. Given a diagram $X\in\D(B)$ by \cite[Lem.~3.10]{groth:revisit} there is a commutative diagram
% \[
% \xymatrix{
% u_!Fu^\ast\ar@{=>}[r]^-\cong\ar@{=>}[d]_-{\gamma^{-1}}^\cong&Fu_!u^\ast\ar@{=>}[d]^-{F\varepsilon}\\
% u_!u^\ast F\ar@{=>}[r]_-{\varepsilon F}&F.
% }
% \]
% in which the unlabeled morphism is the canonical mate expressing the compatibility of $F$ with $u_!$. Since $F$ is assumed to preserve left Kan extensions along $u$, this canonical mate is an isomorphism. Thus, $FX$ lies in the essential image of $u_!\colon\E(A)\to\E(B)$ if and only if $\varepsilon F$ is an isomorphism if and only if $F\varepsilon$ is an isomorphism. Since $F$ is conservative this is the case if and only if $\varepsilon\colon u_! u^\ast X\to X$ is an isomorphism which is to say that $X$ lies in the essential image of $u_!\colon\D(A)\to\D(B)$.
% \end{proof}

% \begin{cor}\label{cor:cons-refl}
% Let $F\colon\D\to\E$ be a conservative morphism of derivators and let $A\in\cCat$. If $F$ preserves colimits of shape $A$, then $F$ reflects colimits of shape $A$.
% \end{cor}
% \begin{proof}
% Since $F$ preserves colimits of shape $A$ if and only if it preserves left Kan extensions along the fully faithful functor $i_A\colon A\to A^\rhd$ (\cite[Prop.~3.9]{groth:revisit}), this statement is immediate from \autoref{lem:cons-refl}.
% \end{proof}

% \begin{cor}\label{cor:adj-refl-colim}

% \begin{enumerate}
% \item \label{cor:adj-refl-colimI} Coreflections of derivators preserve and reflect colimits.
% \item \label{cor:adj-refl-colimII} Reflections of derivators preserve and reflect limits.
% \item \label{cor:adj-refl-colimIII} Equivalences of derivators preserve and reflect limits and colimits.
% \end{enumerate}
% \end{cor}
% \begin{proof}
% This is immediate from \autoref{cor:cons-refl}.
% \end{proof}

% % Because of its relevance in \S\ref{sec:lifting-t}, we explicitly state the following example which is immediate from \autoref{egs:refl-loc}.

% % \begin{egs}\leavevmode\label{eg:lim-coconn}
% % \begin{enumerate}
% % 	\item Let $k\in\lZ$. The full subderivator $\cSp_{\leq k}\subseteq\cSp$ of $k$-coconnective spectra is closed under limits and the full subderivator $\cSp_{\geq k}\subseteq\cSp$ of $k$-connective spectra is closed under colimits. 
% % 	\item Let $E$ be a spectrum. The class of $E$-torsion spectra $\{X \in\cSp\mid X\land E\simeq *\}$ \cite{} is a coreflection of $\cSp$ generated by a single element \cite{}. 
% % 	\item Let $p$ be a prime number. The class of $p$\emph{-acyclic} chain complexes of abelian groups $\{X_\bullet\mid X_\bullet\otimes \mathbf{Z}/p\mathbf{Z}\simeq 0_\bullet\}$ is a coreflection of $\text{Ch}(\mathbf Z)$.
% % \end{enumerate}
% % \end{egs}
% % \fcomment{There's plenty of examples here: Bousfield localization of spectra, $p$-localization of spectra, $p$-localization of complexes, etc. etc.}
% % To conclude this section, in the following remark we collect the compatibilities of reflections and Kan extensions (as a refinement of \autoref{rmk:refl-loc}).

% \begin{rmk}
% Let $L\colon\D\rightleftarrows\E\colon R$ be a reflection of derivators.
% \begin{enumerate}
% \item The left adjoint $L$ preserves left Kan extensions.
% \item The left adjoint $L$ preserves right Kan extensions of diagrams in the essential image of $R$.
% \item The right adjoint $R$ preserves and reflects right Kan extensions.
% \end{enumerate}
% It only remains to verify the second claim, and for that purpose let $u\colon A\to B$ be in $\cCat$. In order to show that the canonical mate $Lu_\ast R\to u_\ast LR$ is invertible, it suffices to consider the following diagram
% \[
% \xymatrix{
% LRu_\ast\ar[r]^-\sim\ar[d]_-\varepsilon^-\sim&Lu_\ast R\ar[r]&u_\ast LR\ar[d]^-\varepsilon_-\sim\\
% u_\ast\ar[rr]_-\id&&u_\ast
% }
% \]
% which commutes by functoriality of canonical mates and \cite[Lem.~3.11]{groth:revisit}.
% \end{rmk}
% % \todo[inline, caption=0]{
% % Possibly relevant left-overs:
% % \begin{enumerate}
% % \item Discuss creation of limits? Motivation: a monadic functor (\autoref{monadic}) creates all limits that exist in the domain. %Derivator Barr-Beck: a functor is monadic iff has a left adjoint, reflects isos, and creates limits of split pairs (see below chapter on monads)
% % \end{enumerate}}
% \begin{defn}\label{creates}
% Let $F : \D \to \E$ be a morphism of prederivators; we say that $F$ \textbf{creates homotopy left} (\textbf{resp., right}) \textbf{Kan extensions along} $u : A\to B$ if for every $X\in \D(B)$, 
% \begin{itemize}
% 	\item the object $X$ lies in the essential image of $u_!^\D$ (resp, $u_*^\D$) if and only if $F_BX$ lies in the essential image of $u_!^\E$ (resp, $u_*^\D$);
% 	\item $F$ preserves homotopy left (resp., right) Kan extensions along $u$.
% \end{itemize}
% \end{defn}
% % \begin{rmk}
% % Note that if $F : \D \to \E$ creates homotopy left/right Kan extensions along $u$ then it also reflects them, and that
% % \todo[inline]{Finish this remark!}
% % \end{rmk}
